Optimal Privacy Preserving for Federated Learning in Mobile Edge Computing

Federated Learning (FL) with quantization and deliberately added noise over wireless networks is a promising approach to preserve user differential privacy (DP) while reducing wireless resources. Specifically, an FL process can be fused with quantized Binomial mechanism-based updates contributed by multiple users. However, optimizing quantization parameters, communication resources (e.g., transmit power, bandwidth, and quantization bits), and the added noise to guarantee the DP requirement and performance of the learned FL model remains an open and challenging problem. This article aims to jointly optimize the quantization and Binomial mechanism parameters and communication resources to maximize the convergence rate under the constraints of the wireless network and DP requirement. To that end, we first derive a novel DP budget estimation of the FL with quantization/noise that is tighter than the state-of-the-art bound. We then provide a theoretical bound on the convergence rate. This theoretical bound is decomposed into two components, including the variance of the global gradient and the quadratic bias that can be minimized by optimizing the communication resources, and quantization/noise parameters. The resulting optimization turns out to be a Mixed-Integer Non-linear Programming (MINLP) problem. To tackle it, we first transform this MINLP problem into a new problem whose solutions are proved to be the optimal solutions of the original one. We then propose an approximate algorithm to solve the transformed problem with an arbitrary relative error guarantee. Extensive simulations show that under the same wireless resource constraints and DP protection requirements, the proposed approximate algorithm achieves an accuracy close to the accuracy of the conventional FL without quantization/noise. The results can achieve a higher convergence rate while preserving users' privacy.

==> deleted-tex.tex <==
	
% 	Considering the formulation (\ref{eq:expression-epsilon}), it is clear that $\epsilon$ is monotonically decreasing over $m$ for any particular value of $l$ and $p$. Therefore, for a particular values set $(\varepsilon}, l, p)$, there is a positive integer $m_{\varepsilon, l, p}$ such that for any $m \geq m_{\varepsilon, l, p}$, the parameter $\epsilon \leq \varepsilon$. In advance, the value $m_{\varepsilon, l, p}$ could be easily computed using a binary algorithm over a feasible interval of $m$. As a result, we could replace the constraint \eqref{eq:eps_cons} by the constraint: $m \geq m_{\varepsilon, l, p}$.

%% BEGIN commented in March 03 2022 P-1
%     \begin{theorem}[Solutvalue $m \geq m_{$ion of $\mathcal{l, p}P }_1$]
%     Let $l_0$ be the maximal integer solution of the inequation $l + \lceil 8/K(l+1)\rceil \leq 2^{TW/d} (1 + \min_{k \in K} P_k^{\max}h_k / N_0)$. The optimal solution of ($\mathscr{P}_1$) is:
    
%     \[
%     l =  \begin{cases}
%     \min\{\lceil \frac{23}{2} \log(\frac{10d}{\delta})\rceil - 2, \lfloor 2^{\frac{TW}{d}} (1 + \frac{\min_{k \in K} P_k^{\max} h_k}{N_0}) \\
%     \quad \quad \quad \quad \quad \quad - \lceil \frac{92}{K} \log(\frac{10d}{\delta})\rceil\rfloor \}, \ \text{if} \ l_0 < \lceil \frac{23}{2} \log(\frac{10d}{\delta})\rceil - 1 \\

%     \arg_{l} \min\{g(l_0), g(\min\{ \lceil \frac{23}{2}\log(\frac{10d}{\delta}) \rceil - 2, \lfloor 2^{\frac{TW}{d}}(1 + \\ 
%     \quad \quad \quad \quad \quad \quad \frac{\min_{k \in K}P_k^{\max} h_k}{N_0}) -  \lceil \frac{92}{K} \log(\frac{10d}{\delta}) \rceil \rfloor \}), \\
%     \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \text{if} \ l_0 \geq \lceil \frac{23}{2} \log(\frac{10d}{\delta})\rceil - 1, 
%     \end{cases}
%     \]
%     where $g(l) = 1 / (l-1)^2 + 4 \max\{23\log(10d / \delta), 2(l+1)\}/ (K (l-1)^2)$, and $m = \lceil 4/K \max\{23 \log(10d / \delta), 2(l + 1)\}\rceil$, $p = p_l$ where $p_l$ is the solution of following quadrtic equation:
%     $$p_l(1-p_l) = \frac{1/K\max\{23\log(\frac{10d}{\delta}), 2(l+1)\}}{\lceil 4/K\max\{23\log(\frac{10d}{\delta}), 2(l+1)\}\rceil}$$
%     and $P_k = \min\{((l + m)2^{d/(TW)} - 1)N_0/h_k, P^{\max}_k\}$.
%     \end{theorem}
%     \begin{proof}
%         The proof is in Appendix \ref{proof-theorem-2}
%     \end{proof}
	
% 	%		\begin{alignat}{3}
% 	%			\max_x              &\quad&  z = \sum_{j=1}^n c_i x_j  &&          & \\
% 	%			\text{s.t: } &\quad&  \sum_{j=1}^n a_{ij} x_j   && \leq b_i &\quad \forall i=1,m\\
% 	%			&\quad&  x_j && \geq 0   &\quad \forall j=1,n
% 	%		\end{alignat}
% 	%	
	
% 	\subsubsection{Minimize convergence time while guaranteeing the differential privacy}
	
% 	The constraint (\ref{eq:14}) only ensures the expression of parameter $\epsilon$ of differential privacy mechanism $\mathcal{M}$ as shown in (\ref{eq:expression-epsilon}). The requirement that $\epsilon \leq \varepsilon$ is not guaranteed. We need to add this requirement to the model ($\mathscr{P}_1$) to ensure the differential privacy and that leads to the following model:
	
% 	\begin{equation}
% 		\mathscr{P}_2: \enspace \underset{l,m,p,P_n}{\mathrm{min.}}\quad \frac{1 + 4p(1-p) m}{(l-1)^2} \label{eq:12}\\
% 	\end{equation}
	
% 	\begin{alignat}{2}
% 	\hskip 1em \textrm{s.t.} \quad   \epsilon \leq \varepsilon \\
% 	\quad 	d\log_2(l+m) &\le TW\log_2(1+ \frac{P_k h_k}{N_0}), \forall k \in K 				\label{eq:13}\\
% 	\quad	Kmp\left(1-p\right)	&\geq max\left\{23\log(\frac{10d}{\delta}),2(l+1)\right\}		\label{eq:14}\\
% 	\quad	P^{min}_k \le P_k &\le P^{max}_k,  \forall k \in K 										\label{eq:15} \\
% 	\quad	l, m &\in N \label{eq:16} \\
% 	\quad	p &\in (0,1)	\label{eq:17}
% 	\end{alignat}
	
% 	\underline{\textbf{A relaxation way of DP requirement}}:
	
% 	App the Cauchy inequality for (\ref{eq:cp-exp}), (\ref{eq:bp-exp}), and (\ref{eq:dp-exp}), we could imply that:
% 	\begin{equation}\frac{7\sqrt{2}}{4} \leq c_p \leq 5\sqrt{2}, \ \frac{2}{3} \leq d_p \leq \frac{4}{3}, \ -\frac{1}{3} \leq b_p \leq \frac{5}{3}. \label{cauchy-est-for-cp-bp-dp} \end{equation}
	
% 	Replace $s = 2M/(l - 1)$ into equations (\ref{eq:Delta_1-1-exp}) and (\ref{eq:Delta_2-1-exp}) we have:
% 	\begin{align}
% 	    \nonumber \Delta_1 & = \frac{2\sqrt{d}M}{\frac{2M}{l - 1}} + \sqrt{\frac{4\sqrt{d}M \log(\frac{2}{\delta})}{\frac{2M}{l - 1}}} + \frac{4}{3} \log \left( \frac{2}{\delta} \right) \\
% 	    & = \sqrt{d}(l - 1) + \sqrt{2\sqrt{d}(l - 1)\log \left(\frac{2}{\delta}\right)} + \frac{4}{3} \log \left( \frac{2}{\delta} \right) \label{eq:Delta_1-by-l}
% 	\end{align}
% 	\begin{align}
% 	    	\nonumber \Delta_2  & = \frac{2M}{\frac{2M}{l - 1}} + \sqrt{\Delta_1 + \sqrt{\frac{4\sqrt{d}M\log\left(\frac{2}{\delta}\right)}{\frac{2M}{l - 1}}}} \\
% 	    	& = (l - 1) + \sqrt{\Delta_1 + \sqrt{2\sqrt{d}(l - 1) \log \left(\frac{2}{\delta}\right)}} \label{eq:Delta_2-by-l}
% 	\end{align}
	
% 	Combining (\ref{cauchy-est-for-cp-bp-dp}), (\ref{eq:Delta_1-by-l}), and (\ref{eq:Delta_1-by-l}) consequences that:
% 	\begin{align}
% 	\nonumber \epsilon & = \frac{\Delta_2 \sqrt{2 \log \frac{1.25}{\delta}}}{s\sqrt{mp(1-p)}} + \frac{\Delta_2 c_p \sqrt{\log \frac{10}{\delta}} + \Delta_1 b_p} {smp(1-p)(1-\frac{\delta}{10})} \\
% 	\nonumber & \quad \ + \frac{\frac{2}{3}\Delta_\infty \log\frac{1.25}{\delta} + \Delta_\infty d_p \log\frac{20d}{\delta} \log\frac{10}{\delta}} {smp(1-p)} \\
% 	\nonumber & \leq \frac{\Delta_2 \sqrt{2 \log \frac{1.25}{\delta}}}{\frac{2M}{l - 1} \sqrt{\frac{23}{K} \log\left( \frac{10d}{\delta} \right)}} + \frac{\Delta_2 5\sqrt{2} \sqrt{\log \frac{10}{\delta}} + \Delta_1 \frac{5}{3}}{\frac{2M}{l - 1} \frac{23}{K} \log \left( \frac{10d}{\delta} \right) \left( 1 - \frac{\delta}{10}\right)} + \\
% 	\nonumber &\quad \ \frac{\frac{2}{3} (l + 1) \log \frac{1.25}{\delta} + (l + 1) \frac{4}{3} \log \frac{20d}{\delta} \log \frac{10}{\delta}}{\frac{2M}{l - 1}2(l + 1)} \\
% 	\nonumber & = \frac{\Delta_2 (l - 1)}{2M} \left( \sqrt{\frac{2K \log \frac{1.25}{\delta}}{23 \log \frac{10d}{\delta}}} + K \frac{5\sqrt{2} \sqrt{\log \frac{10}{\delta}}}{23 \log \frac{10d}{\delta} (1 - \frac{\delta}{10})}\right) \\
% 	\nonumber  & \quad \ + \Delta_1(l - 1) \frac{5K}{138 M \log \frac{10d}{\delta} \left( 1 - \frac{\delta}{10}\right)} \\
% 	& \quad \  + (l - 1)\frac{\log \frac{1.25}{\delta} + 2 \log \frac{20d}{\delta} \log \frac{10}{\delta}}{6M} = \xi(l).
% 	\end{align}
	
% 	It is clear that $\xi(l)$ is a strickly monotonic function on $l$. As a result, the equation $\xi(l) = \varepsilon$ could be solved easily using any approximation method, e.g. the binary search. Therefore, instead of directly considering $\epsilon \leq \varepsilon$, we could consider $\epsilon \leq \xi(l) \leq \varepsilon$. This inequality leads to the the constraint $l \leq \xi^{-1}(\varepsilon)$, where $\xi^{-1}(\varepsilon)$ is the solution of equation $\xi(l) = \varepsilon$.
	
% 	Hence, the model that guarantee two targets: optimizing the convergence time and guaranteeing the differential privacy parameter $\epsilon$ is presented as following:
	
% 	\begin{equation}
% 		\mathscr{P}_3: \enspace \underset{l,m,p,P_n}{\mathrm{min.}}\quad \frac{1 + 4p(1 - p)m}{(l-1)^2} \label{eq:convegence-gurantee-dp-12}\\
% 	\end{equation}
	
% 	\begin{alignat}{2}
% 	\hskip 1em \textrm{s.t.} \ 
% 	l \leq \xi^{-1}(\varepsilon),\\
% 	\quad 	d\log_2(l+m) &\le TW\log_2(1+ \frac{P_k h_k}{N_0}), \forall k \in K 				\label{eq:convegence-gurantee-dp-13}\\
% 	\quad	Kmp\left(1-p\right)	&\geq max\left\{23\log(\frac{10d}{\delta}),2(l+1)\right\}		\label{eq:convegence-gurantee-dp-14}\\
% 	\quad	P^{min}_k \le P_k &\le P^{max}_k,  \forall k \in K 										\label{eq:convegence-gurantee-dp-15} \\
% 	\quad	l, m &\in N \label{eq:convegence-gurantee-dp-16} \\
% 	\quad	p &\in (0,1)	\label{eq:convegence-gurantee-dp-17}
% 	\end{alignat}
	
% 	The solution of Model ($\mathscr{P}_2$) is presented in the following theorem.
	
% 	\begin{theorem}[Solution of ($\mathscr{P}_2$)]\label{theorem-sol-of-P2}
%     Let $l_0$ be the maximal integer solution of the inequation $l + \lceil 8/K(l+1)\rceil \leq 2^{TW/d} (1 + \min_{k \in K} P_k^{\max}h_k / N_0)$. The optimal solution of ($\mathscr{P}_2$) is:
    
%     \[
%     l =  \begin{cases}
%     \min\{\lceil \frac{23}{2} \log(\frac{10d}{\delta})\rceil - 2, \lfloor 2^{\frac{TW}{d}} (1 + \frac{\min_{k \in K} P_k^{\max} h_k}{N_0}) - \\
%     \lceil \frac{92}{K} \log(\frac{10d}{\delta})\rceil\rfloor, \lfloor \xi^{-1}(\varepsilon) \rfloor \}, \ \text{if} \ \lfloor \xi^{-1}(\varepsilon) \rfloor < \lceil \frac{23}{2} \log(\frac{10d}{\delta})\rceil \\
%     - 1, \text{or} \ \lfloor \xi^{-1}(\varepsilon) \rfloor \geq \lceil \frac{23}{2} \log(\frac{10d}{\delta})\rceil - 1 \ \text{and} \ l_0 < \\
%     \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \ \ \ \lceil \frac{23}{2} \log(\frac{10d}{\delta})\rceil - 1, \\
    
%     \arg_{l} \min\{g(\min\{l_0, \lfloor \xi^{-1}(\varepsilon)\rfloor \}), g(\min\{ \lceil \frac{23}{2}\log(\frac{10d}{\delta}) \rceil \\
%     - 2, \lfloor 2^{\frac{TW}{d}}(1 + \frac{\min_{k \in K}P_k^{\max} h_k}{N_0}) -  \lceil \frac{92}{K} \log(\frac{10d}{\delta}) \rceil \rfloor \}), \\
%     \text{if} \ \lfloor \xi^{-1}(\varepsilon) \rfloor \geq \lceil \frac{23}{2} \log(\frac{10d}{\delta})\rceil - 1 \ \text{and} \ l_0 \geq \lceil \frac{23}{2} \log(\frac{10d}{\delta})\rceil\\
%     \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \ \ \ - 1, 
%     \end{cases}
%     \]
%     where $g(l) = 1 / (l-1)^2 + 4 \max\{23\log(10d / \delta), 2(l+1)\}/ (K(l-1)^2)$, and $m = \lceil 4/K \max\{23 \log(10d/\delta), 2(l + 1)\}\rceil$, $p = p_l$ where $p_l$ is the solution of following quadrtic equation:
%     $$p_l(1-p_l) = \frac{1/K\max\{23\log(\frac{10d}{\delta}), 2(l+1)\}}{\lceil 4/K\max\{23\log(\frac{10d}{\delta}), 2(l+1)\}\rceil}$$
%     and $P_k = \min\{((l + m)2^{d/TW} - 1)N_0/h_k, P^{\max}_k\}$.
%     \end{theorem}
%     \begin{proof}
%         The proof of this theorem is analogically with the proof in Appendix \ref{proof-theorem-2}.
%     \end{proof}

% n pra    && \xi^{-1}(\varepsilon).

% ctice, we observe that $23 \log(10d/\delta)$ is often far larger than $2(l +1)$, $l_0$ and . Therefore, we could apply a reduced form of the solution presented in Theorem $\ref{theorem-sol-of-P2}$ as following:
%     \begin{align*}l \ & = & \min\{\lfloor 2^{\frac{TW}{d}} (1 + \frac{\min_{k \in K} P_k^{\max} h_k}{N_0}) - \lceil \frac{92}{K} \log(\frac{10d}{\delta})\rceil\rfloor, \\
%     && \lfloor \xi^{-1}(\varepsilon) \rfloor\}.\end{align*}
    
%     To solve the equation ...... is very hard. We apply another approach 
	
% 	\underline{\textbf{A discrete way to ensure DP requirement}}:
	
% 	Another approximation way to solve the model ($\mathscr{P}_2$) is described as following. We limit the investigation on the value of $l$ on the interval $[5, 127]$. For each value of $l$, we find the real value $\rho_l$ such that for any $mp(1-p) \geq \rho_l$ the following inequality is satisfied: $\epsilon \leq \varepsilon$. Since the $\epsilon$ is in the reverse relationship with $mp(1- p)$, this could be done by applying the binary search algorithm on a range for $mp(1-p)$. In this problem, we set the search range for $mp(1-p)$ as $[1, 2^{26} - 1]$. We build a discrete feasible solution set $\mathcal{S}$ for $(l, m, p)$ as following: For each pair of $(l, p) \in [5, 127] \times \{0.01, 0.02, \ldots, 0.99\}$ we compute: $m = \lceil \rho_l / (p(1 - p))\rceil$. We then compute the objective function of ($\mathscr{P}_2$) on $S$ and output the minimum solution.
%% END commented in March 03 2022 P-1

	% An example of a floating figure using the graphicx package.
	% Note that \label must occur AFTER (or within) \caption.
	% For figures, \caption should occur after the \includegraphics.
	% Note that IEEEtran v1.7 and later has special internal code that
	% is designed to preserve the operation of \label within \caption
	% even when the captionsoff option is in effect. However, because
	% of issues like this, it may be the safest practice to put all your
	% \label just after \caption rather than within \caption{}.
	%
	% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
	% option should be used if it is desired that the figures are to be
	% displayed while in draft mode.
	%
	%\begin{figure}[!t]by
	%\centering
	%\includegraphics[width=2.5in]{myfigure}
	% where an .eps filename suffix will be assumed under latex, 
	% and a .pdf suffix will be assumed for pdflatex; or what has been declared
	% via \DeclareGraphicsExtensions.
	%\caption{Simulation results for the network.}
	%\label{fig_sim}
	%\end{figure}
	
	% Note that the IEEE typically puts floats only at the top, even when this
	% results in a large percentage of a column being occupied by floats.
	% However, the Computer Society has been known to put floats at the bottom.
	
	
	% An example of a double column floating figure using two subfigures.
	% (The subfig.sty package must be loaded for this to work.)
	% The subfigure \label commands are set within each subfloat command,
	% and the \label for the overall figure must come after \caption.
	% \hfil is used as a separator to get equal spacing.
	% Watch out that the combined width of all the subfigures on a 
	% line do not exceed the text width or a line break will occur.
	%
	%\begin{figure*}[!t]
	%\centering
	%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
	%\label{fig_first_case}}
	%\hfil
	%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
	%\label{fig_second_case}}
	%\caption{Simulation results for the network.}
	%\label{fig_sim}
	%\end{figure*}
	%
	% Note that often IEEE papers with subfigures do not employ subfigure
	% captions (using the optional argument to \subfloat[]), but instead will
	% reference/describe all of them (a), (b), etc., within the main caption.
	% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
	% labels, the optional argument to \subfloat must be present. If a
	% subcaption is not desired, just leave its contents blank,
	% e.g., \subfloat[].
	
	
	% An example of a floating table. Note that, for IEEE style tables, the
	% \caption command should come BEFORE the table and, given that table
	% captions serve much like titles, are usually capitalized except for words
	% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
	% and up, which are usually not capitalized unless they are the first or
	% last word of the caption. Table text will default to \footnotesize as
	% the IEEE normally uses this smaller font for tables.
	% The \label must come after \caption as always.
	%
	%\begin{table}[!t]
	%% increase table row spacing, adjust to taste
	%\renewcommand{\arraystretch}{1.3}
	% if using array.sty, it might be a good idea to tweak the value of
	% \extrarowheight as needed to properly center the text within the cells
	%\caption{An Example of a Table}
	%\label{table_example}
	%\centering
	%% Some packages, such as MDW tools, offer better commands for making tables
	%% than the plain LaTeX2e tabular which is used here.
	%\begin{tabular}{|c||c|}
	%\hline
	%One & Two\\
	%\hline
	%Three & Four\\
	%\hline
	%\end{tabular}
	%\end{table}
	
	
	% Note that the IEEE does not put floats in the very first column
	% - or typically anywhere on the first page for that matter. Also,
	% in-text middle ("here") positioning is typically not used, but it
	% is allowed and encouraged for Computer Society conferences (but
	% not Computer Society journals). Most IEEE journals/conferences use
	% top floats exclusively. 
	% Note that, LaTeX2e, unlike IEEE journals/conferences, places
	% footnotes above bottom floats. This can be corrected via the
	% \fnbelowfloat command of the stfloats package.
	
% 	By solving equation $\xi(l) = \varepsilon$, we have an imagination about the relation between level quantization $l$ and differential privacy parameter $\epsilon$. We set the upper bound $\varepsilon$ at different values: 10, 100, 1000, 10000, 100000 and compute the upper bound $\xi^{-1}(\varepsilon)$. As a result, we receive the chart shown in Figure \ref{upper-bound-l-over-log-10-of-epsilon}.

   % }

%%%% BEGIN comment on 10/03/2022 P-3
% 	\begin{figure}[b]
% 		\centerline{\includegraphics[width=0.55\textwidth]{figures/upper-bound-l-over-log-10-of-epsilon.png}}
% 		\caption{Upper bound on level quantization vs the upper bound on epsilon with number of devices $K = 100$}
% 		\label{upper-bound-l-over-log-10-of-epsilon}
% 	\end{figure}
	
% 	The chart in Figure \ref{upper-bound-l-over-log-10-of-epsilon} shows that, as the upper bound of the differential privacy's parameter $\epsilon$ increases, the upper bound for level quantization $l$ also increases. In generality, as the level quantization increases, the convergence speed is faster. This is reasonable.

%     The following chart compare the running time in the case of optimal solution with $l = 3$ and a feasible solution with $l = 2$ with the differential privacy parameter $\epsilon = 10$. The parameters of binomial mechanism are as following: $m = 12$, $p = 0.35607$. As can be seen, in the case of optimal solution, the learning process are conversed at a faster rate.
    
%     \begin{figure}[b]
% 		\centerline{\includegraphics[width=0.55\textwidth]{figures/level-quantization-vs-accuracy.png}}
% 		\caption{Number of rounds}
% 		\label{number-of-rounds-vs-level-quantization}
% 	\end{figure}
	
% 	The chart in Figure \ref{mp1p-over-epsilon} shows the relation between $\epsilon$ and value of $mp(1 - p)$. For each value of $\epsilon$ in $[4, 100]$, we compute the feasible solutions $(l, m, p)$ of model ($\mathscr{P}_2$) corresponding to $l \in [4, 127]$ and $p \in \{0.1, 0.15, \ldots, 0.95\}$. Then we take average value of $mp(1 - p)$ over these solutions to put into the chart. It is easy to see that as $\epsilon$ increases, the average value of $mp(1 - p)$ decreases.
	
% 	\begin{figure}[b]
% 		\centerline{\includegraphics[width=0.5\textwidth]{figures/mp1p-over-epsilon.png}}
% 		\caption{Average of values $mp(1-p)$ over $\epsilon$}
% 		\label{mp1p-over-epsilon}
% 	\end{figure}
	
% 	We intends to make a chart that show the relation between the convergence time and $mp(1 - p)$ of feasible solutions fixing all the input parameters. We do believe that $mp(1 - p)$ has a significant impact on the convergence speed of learning algorithm. It is meaning to note that $mp(1 - p)$ is the variance of the binomial distribution.
%%%% END comment on 10/03/2022 P-3


%% BEGIN commented in March 03 2022 P-2	
% 	\section{Proof of Theorem 2}
% 	\label{proof-theorem-2}
% 	\textbf{1.} We denote the objective function of problem ($\mathscr{P}_1$) as $f(l, m, p, P_k)$. Constraints (\eqref{eq:13}) and (\ref{eq:15}) imply that:
% $$d \log_2(l+m) \leq TW \log_2(1 + \frac{P^{\max}_k h_k}{N_0}), \ \forall k \in K.$$

% The values of variables $P_k$ are not counted in the objective function $f(l, m, p, P_k)$, but they define the domains of other variables $l$, $m$, $p$. We could consider only case $P_k = P^{\max}_k$ where the domains of $l$, $m$ and $p$ are maximal. In other hand, the left sides of constraints (\ref{eq:13}) are the same. We could replace constraints (\ref{eq:13}) by considering the minimal value of $P_k^{max}h_k/N_0$ among $k \in K$. Hence, the optimal solution of initial problem is equivalent to the optimal solution of the following problem:

% \begin{equation}
% 	\mathscr{P}_{1.1}: \enspace \underset{l, m, p}{\mathrm{min.}} \quad \frac{1 + 4mp(1- p)}{(l-1)^2} \\
% \end{equation}

% \begin{alignat}{2}
% 	\hskip 1em \textrm{s.t.} \ d\log_2(l+m) \leq TW \log_2 \left(1 + \frac{\min_{k \in K}(P^{\max}_k h_k)}{N_0} \right) \label{power-bandwidth-constraint-prior-model-m2}\\
%     \quad Kmp(1-p) \geq \max\{23\log(\frac{10d}{\delta}), 2(l+1)\} \label{DP-constraint-prior-model-m2}\\
%     \quad l, m \in N \\
%     \quad p \in (0, 1),
% \end{alignat}

% For the sake of convenience, we denote the objective function of ($\mathscr{P}_{1.1}$) as $f(l, m, p)$.

% \textbf{2.} Apply Cauchy inequality, it is clear that: $0 < p(1-p) \leq 1/4$ for $p \in (0, 1)$. Therefore, we have: $Km/4 \geq Kmp(1-p)$. This combines with constraint (\ref{DP-constraint-prior-model-m2}) lead to the following consequence: $Km/4 \geq \max\{23\log(10d/\delta), 2(l+1)\}$, which is equivalent to $m \geq 4/K\max\{23\log(10d/\delta), 2(l+1)\}$. Since $m$ is an integer, we have: $m \geq \lceil 4/K\max\{23\log(10d/\delta), 2(l+1)\}\rceil$, where $\lceil \cdot \rceil$ is the ceiling function.

% We notice that the equation $x(1-x) = a$ always has a solution $x \in (0, 1)$ for every parameter $0 < a \leq 1/4$. It is clear that 
% $$0 < \frac{1/K\max\{23\log(\frac{10d}{\delta}), 2(l+1)\}}{\lceil 4/K \max\{23\log(\frac{10d}{\delta}), 2(l+1)\}\rceil} \leq \frac{1}{4},$$ since $0 < x/\lceil 4x \rceil \leq 1/4$ for every $x > 0$. Consequently, for any $l$, there is always a value $p_l \in (0, 1)$ such that:
% \begin{align}
% p_l(1-p_l) = \frac{1/K \max\{23\log(\frac{10d}{\delta}), 2(l+1)\}}{\lceil 4/K \max\{23\log(\frac{10d}{\delta}), 2(l+1)\}\rceil}.
% \end{align}\label{quad-equa-p} Hence, if $(l_0, m_0, p_0)$ is a feasible solution of ($\mathscr{P}_2$), then $(l_0, \lceil 4/K \max\{23\log(10d/\delta), 2(l_0+1)\}\rceil, p_{l_0})$ is also a feasible solution of problem ($\mathscr{P}_{1.1}$).   

% Apply constraint (\eqref{DP-constraint-prior-model-m2}) to the objective function, we have:
% \begin{multline*}
% f(l_0, m_0, p_0) = \frac{1 + 4 m_0 p (1 - p)}{(l_0-1)^2}
% \\
% \geq f(l_0, \lceil 4/K\max\{23\log(\frac{10d}{\delta}), 2(l_0+1)\}\rceil, p_{l_0})\\
% = \frac{1}{(l_0-1)^2} + \frac{4 \max\{23\log(\frac{10d}{\delta}), 2(l_0+1)\}}{K(l_0-1)^2}
% \end{multline*}

% Thus we could narrow the solution search's space by considering only the case $m = \lceil 4/K\max\{23\log(10d/\delta), 2(l+1)\}\rceil$ and $p = p_l$.

% As a result, we imply that the optimal solution of problem ($\mathscr{P}_{1.1}$) is equivalent to the optimal solution of the following problem:

% \begin{equation}
% 	\mathscr{P}_{1.2}: \enspace \underset{l}{\mathrm{min.}} \ \frac{1}{(l-1)^2} + \frac{4 \max\{23\log(\frac{10d}{\delta}), 2(l+1)\}}{K(l-1)^2} \label{obj-prior-model-m3}\\
% \end{equation}

% \begin{alignat}{2}
% 	\hskip 1em \textrm{s.t.} \ d \log_2(l+\lceil 4/K\max\{23\log(\frac{10d}{\delta}), 2(l+1)\}\rceil) \leq \nonumber\\
%     \quad \quad \quad TW \log_2 \left(1 + \frac{\min_{k \in K} (P^{\max}_k h_k)}{N_0} \right), \ \forall k \in K\label{power-bandwidth-constraint-pri+or-model-m3}\\
%     l \in N.
% \end{alignat}

% \textbf{3.} Denote the objective function of problem ($\mathscr{P}_{1.2}$) as $g(l)$. Now considering $\max\{23\log(10d/\delta), 2(l+1)\}$, there are two cases:

% \textit{Case 1}: $2(l+1) = \max\{23\log(10d/\delta), 2(l+1)\}$, which is equivalent to $l \geq \lceil (23/2)\log(10d/\delta) - 1\rceil$. In this case, 
% \begin{align*}
%     g(l) & = \frac{1}{(l-1)^2} + \frac{8 (l+1)}{K(l-1)^2} \\
%     & = \frac{K + 8l + 8}{K(l-1)^2}.
% \end{align*} 
% Take the first order derivative of $g(l)$, we have:

% \begin{align*}
% g^{(1)}(l) & = \frac{\left(8(l-1)^2 - (8l + 8 + K)2(l-1)\right)}{K(l-1)^4} \\
% & = \frac{2 (4l - 4 - 8l - 8 - K)}{K(l-1)^3} \\
% & = \frac{2 (-4l - 12 - K)}{K(l-1)^3} < 0, \  \forall l \in N^*.
% \end{align*}

% It is clear that $g(l)$ is a decreased function on $N^*$. Therefore, in \textit{Case 1}, the minimum solution of problem $(\mathscr{P}_{1.2})$ is the maximal integer value $l$ that satisfies the constraints (\ref{power-bandwidth-constraint-prior-model-m2}): $d\log_2(l+\lceil 8/K(l+1)\rceil) \leq TW \log_2(1 + \min_{k \in K} P^{\max}_k h_k/N_0), \ \forall k \in K$ or $l+\lceil 8/K(l+1)\rceil \leq 2^{TW/d}(1 + \min_{k \in K}P^{\max}_k h_k/N_0)$. This integer inequation could be solved easily, and we denote its maximal integer solution as $l_0$ (this is a little abuse of notation). Notice that, if $l_0 < 23/2\log(10d/\delta) - 1$, then this case would never occurs.

% \textit{Case 2}: $23\log(10d/\delta) = \max\{23\log(10d/\delta), 2(l+1)\}$, which implies that $l \leq \lceil 23/2\log(10d/\delta)\rceil - 2$. In this case, 
% \begin{align*}
%     g(l) & = \frac{1}{(l-1)^2} + \frac{92 \log(\frac{10d}{\delta})}{K(l-1)^2}.
% \end{align*} 
% This function is decreased as $l$ is increased.

% Considering constraint (\ref{power-bandwidth-constraint-pri+or-model-m3}), we have:
% $$d\log_2(l + \lceil +\frac{92}{K} \log(\frac{10d}{\delta})\rceil) \leq TW \log_2(1 + \frac{\min_{k \in K} (P_k^{\max}h_k)}{N_0}),$$
% this leads to:
% $$l \leq \lfloor 2^{\frac{TW}{d}} (1 + \frac{\min_{k \in K}P_k^{\max} h_k}{N_0}) -  \lceil \frac{92}{K} \log(\frac{10d}{\delta}) \rceil \rfloor.$$

% We have:
% \begin{align*}
% l \leq & \min\{\lceil \frac{23}{2} \log(\frac{10d}{\delta}) \rceil - 2,\\ 
% & \lfloor 2^{\frac{TW}{d}} (1 + \frac{\min_{k \in K}P_k^{\max} h_k}{N_0}) -  \lceil \frac{92}{K} \log(\frac{10d}{\delta}) \rceil \rfloor\},
% \end{align*}
% hence in this case, the optimal solution is:
% \begin{align*}
% l = & \min\{\lceil \frac{23}{2} \log(\frac{10d}{\delta}) \rceil - 2,\\ 
% & \lfloor 2^{\frac{TW}{d}} (1 + \frac{\min_{k \in K}P_k^{\max} h_k}{N_0}) -  \lceil \frac{92}{K} \log(\frac{10d}{\delta}) \rceil \rfloor\}.
% \end{align*}

% \textbf{4.} Finally, we conclude about the solution of ($\mathscr{P}_1$):
% \begin{itemize}
%   \item If $l_0$ is smaller than $\lceil 23/2\log(10d/\delta)\rceil - 1$, only \textit{Case 2} could happen. We take $l = \min\{\lceil 23/2 \log(10d/\delta) \rceil - 2, 
% & \lfloor 2^{TW/d} (1 + \min_{k \in K}P_k^{\max} h_k/N_0) - \lceil 92/K \log(10d/\delta) \rceil \rfloor\}$.
%   \item If $l_0$ is not smaller than $\lceil 23/2\log(10d/\delta)\rceil - 1$, both \textit{Case 1} and \textit{Case 2} could occur. We set value of $l$ be one of two choices $l_0$ (\textit{Case 1}) and $\min\{ \lceil 23/2\log(10d/\delta) \rceil - 2, \lfloor 2^{TW/d}(1 + \min_{k \in K}P_k^{\max} h_k/N_0) -  \lceil 92/K \log(10d/\delta) \rceil \rfloor \}$ (\textit{Case 2}) that makes the objective function $g(l)$ smaller.
%   \item For the other variables: $m = \lceil 4/K \max \{23 \log(10d/\delta), 2(l + 1)\}\rceil$, $p = p_l$ - the solution of equation (\ref{quad-equa-p}) and $P_k = \min\{((l + m)^{d/TW} - 1)N_0/h_k, P^{\max}_k\}$ (To save energy we set $P_k$ be the smaller value among $((l + m)2^{d/(TW)} - 1)N_0/h_k$ and $P^{\max}_k$, for $k \in K$).
% \end{itemize}
%% END commented in March 03 2022 P-1

% Therefore, on the domain $[1, +\infty)$, $d\epsilon / dt$ either changes its sign one time from plus to minus or remains minus. As a sequence, the function $\epsilon(t)$ either monotonically increases on $[1, t_0)$ then monotonically decreases on $(t_0, +\infty)$ if there exists such $t_0 \geq 1$ that $d\epsilon / dt (t_0) = 0$, or monotonically decreases on $[1, +\infty)$. Therefore, for any $\epsilon$'s upper bound $\bar{\epsilon}$, there exist $m$ such integers $m_1$, $m_2$, and $m_3$ that, for $m \in [m_1, m_2] \cup [m_3, +\infty)$ we have $\epsilon(m) \leq \bar{\epsilon}$ as explained in Figure ...... That is the statement shown in Theorem \ref{theorem:domain-of-m-satis-eps}.

\begin{algorithm}
	    \caption{Algorithm of value set $m$ s.t. $\epsilon \leq \bar{\epsilon}$}
	    \label{alg:m-epsilon-domain}
	    \begin{flushleft}
	        \hspace*{\algorithmicindent} \textbf{Input}: $l$, $p$, and $\bar{\epsilon}$\\
	        \hspace*{\algorithmicindent} \textbf{Output}: $m_1$, $m_2$, and $m_3$
	    \end{flushleft}
	    \begin{algorithmic}[1]
	        \IF{$(d\epsilon / dt)(\sqrt{2}) > 0$}
	            \STATE $t_U \leftarrow \sqrt{2}$
	            \WHILE{$(d\epsilon / dt)(t_U) > 0$}
	                \STATE $t_U \leftarrow t_U \times \sqrt{2}$
	            \ENDWHILE
	            \STATE $t_L \leftarrow \sqrt{2}$, $t_0 \leftarrow \sqrt{\frac{t_L ^2+ t_U^2}{2}}$
	            \WHILE{$(d\epsilon / dt)(t_0) \neq 0$}
	                \IF{$(d\epsilon / dt)(t_0) > 0$}
	                    \STATE $t_L \leftarrow t_0$, $t_0 \leftarrow \sqrt{(t_L^2 + t_U^2) / 2}$
	                \ELSE
	                    \STATE $t_U \leftarrow t_0$, $t_0 \leftarrow \sqrt{(t_L^2 + t_U^2) / 2}$
	                \ENDIF
	            \ENDWHILE
	            \IF{$\epsilon(t_0) > \bar{\epsilon}$}
	                \STATE $m_1 \leftarrow \sqrt{2}$, $t_L \leftarrow \sqrt{2}$, $t_U \leftarrow t_0$, $t_2 \leftarrow \sqrt{(t_L^2 + t_U^2) / 2}$
	                \WHILE{$\epsilon(t_2) \neq \bar{\epsilon}$}
	                    \IF{$\epsilon(t_2) > \bar{\epsilon}$}
	                        \STATE $t_U \leftarrow t_2$, $t_2 \leftarrow \sqrt{(t_L^2 + t_U^2) / 2}$
	                   \ELSE
	                        \STATE $t_L \leftarrow t_2$, $t_2 \leftarrow \sqrt{(t_L^2 + t_U^2) / 2}$
	                    \ENDIF
	                \ENDWHILE
	                \STATE $m_2 \leftarrow (t_2)^2$, $t_L \leftarrow t_0$, $t_U \leftarrow t_0$
	                \WHILE{$\epsilon(t_U) > \bar{\epsilon}$}
	                    \STATE $t_U \leftarrow t_U \times \sqrt{2}$
	                \ENDWHILE
	                \STATE $t_3 \leftarrow \sqrt{(t_L^2 + t_U^2) / 2}$
	                \WHILE{$\epsilon(t_3) \neq \bar{\epsilon}$}
	                    \IF{$\epsilon(t_3) > \bar{\epsilon}$}
	                        \STATE $t_L \leftarrow t_3$, $t_3 \leftarrow \sqrt{(t_L^2 + t_U^2) / 2}$
	                   \ELSE
	                        \STATE $t_U \leftarrow t_3$, $t_3 \leftarrow \sqrt{(t_L^2 + t_U^2) / 2}$
	                    \ENDIF
	                \ENDWHILE
	                \STATE $m_3 \leftarrow (t_3)^2$
	            \ELSE
	                \STATE $m_1 \leftarrow 2$, $m_2 \leftarrow 2$, $m_3 \leftarrow 2$
	            \ENDIF
	        \ELSE
	            \IF{$\epsilon(\sqrt{2}) \leq \bar{\epsilon}$}
	                \STATE $m_1 \leftarrow 2$, $m_2 \leftarrow 2$, $m_3 \leftarrow 2$
	            \ELSE
	                \STATE $t_U \leftarrow \sqrt{2}$
	                \WHILE{$\epsilon(t_U) > \bar{\epsilon}$}
	                    \STATE $t_U \leftarrow t_U \times \sqrt{2}$
	                \ENDWHILE
	                \STATE $t_L \leftarrow \sqrt{2}$, $t_1 \leftarrow \sqrt{(t_L^2 + t_U^2) / 2}$
	                \WHILE{$\epsilon(t_1) \neq \bar{\epsilon}$}
	                    \IF{$\epsilon(t_1) > \bar{\epsilon}$}
	                        \STATE $t_L \leftarrow t_1$, $t_1 \leftarrow \sqrt{(t_L^2 + t_U^2) / 2}$
	                    \ELSE
	                        \STATE $t_U \leftarrow t_1$, $t_1 \leftarrow \sqrt{(t_L^2 + t_U^2) / 2}$
	                    \ENDIF
                    \ENDWHILE
                    \STATE $m_1 \leftarrow (t_1)^2$, $m_2 \leftarrow (t_1)^2$ , $m_3 \leftarrow (t_1)^2$
	            \ENDIF
	        \ENDIF
	   \RETURN $m_1$, $m_2$, $m_3$
	    \end{algorithmic}
	\end{algorithm}
	
	\begin{theorem} \label{theorem:domain-of-m-satis-eps}
	    For a particular values set $(\bar{\epsilon}, l, p)$ if there exists positive integer $m$ such that $\epsilon(m) \leq \bar{\epsilon}$ then there exist integers $0 < m_1 \leq m_2 \leq m_3$ such that, for any $m$ in union of intervals $[m_1, \ m_2]$ and $[m_3, \ +\infty)$ then, $\epsilon(l, m, p) \leq \bar{\epsilon}$. 
	\end{theorem}
	

	\subsubsection{A particular case}
	%% A paragraph about the hardness of problem.
	The model ($\mathscr{P}_2$) is very hard to correctly solve. Therefore, we will investigate the solution in a particular case of this model before getting deeper in a general solution.
	
	Appearing in the objective function, the parameter $G$ that was defined as the upper bound of the gradient of loss function $\Vert \nabla F(w^t) \Vert^2 \le G$ could be set as a constant. This is due to the difficulty of the precise value estimation for $G$. In other hand, we set the maximum value $M$ of quantization scheme equalling to $G$: $M = G$ and apply clipping in distributed learning scheme. Therefore, we could also write $G = s(l - 1) / 2$ since the noise scale is defined as $s = 2M / (l - 1)$. In this situation, we could investigate a class of feasible solutions of model ($\mathscr{P}_1$) which have the same value of $s$. In this particular case, we replace $G = s(l - 1) / 2$ into the objective function of ($\mathscr{P}_1$), then remove the constants away. We receive the new objective function as following,
	$$p(1 - p)m.$$
	
	Considering the particular value of $p$ in the case $s$ is constant, $\epsilon$ is monotonically increasing over $l$ and monotonically decreasing over $m$. The smaller value of $l$ thus leads to the smaller value of $m_{\bar{\epsilon}, l, p}$. Applying constraint \eqref{eq:value_m}, this also leads to possible smaller value of $m$ and loosen the constraint \eqref{eq:channel_cap_cons_in_m}. On the other hand, the objective function in this case as $mp(1- p)$ is monotonically decreasing over $m$. As a sequence, for fixed value of $p$, we could set value of $l$ as least as possible and compute $m$ by equation \eqref{eq:value_m}. In practise, we could set $l = 2$.
	
    We shall present the dependence between variables $m$, $l$ and $p$. We consider the parameter $\epsilon$ computed by (\ref{eq:expression-epsilon}) as a mono-variable function of $m$ for a particular value of $l$ and $p$. For convenience, we also relax the integer type condition of $m$ and consider $m$ in positive real set $\mathbb{R}^+$.
    
    \begin{figure}[b]
		\centerline{\includegraphics[width=0.50\textwidth]{figures/Accuracies-vs-ObjFuncValue-vary-noise-scale.png}}
		\caption{Accuracy vs objective value with noise scale $s = 1$}
		\label{Accuracies-vs-ObjFuncValue-vary-noise-scale}
	\end{figure}
    
    Intending charts:
    % \text{\color{red}
    \begin{enumerate}
        \item A chart of objective value and best accuracy fixing $s = 4$, $\bar{\epsilon} = 4$, $l \in \{2^{\alpha x + \beta} | x \in [1, 1000], \alpha + \beta = 2, 1000 \alpha + \beta = \log{157.938.837}\}$, $p \in \{0.01, 0.02, \ldots, 0.99\}$.
        \item A chart of objective value and best accuracy fixing $s = 1$, $\bar{\epsilon} = 4$, $l \in \{2^{\alpha x + \beta} | x \in [1, 1000], \alpha + \beta = 2, 1000 \alpha + \beta = \log{157.938.837}\}$, $p \in \{0.01, 0.02, \ldots, 0,99\}$. Discussion: As shown in Figure \ref{Accuracies-vs-ObjFuncValue-vary-noise-scale}, the accuracy tends to improve as the objective function value of Problem $\mathscr{P}_3$ decreases.
        \item A chart of objective value and best accuracy fixing $s = 0.1$, $\bar{\epsilon} = 4$, $l \in \{2^{\alpha x + \beta} | x \in [1, 1000], \alpha + \beta = 2, 1000 \alpha + \beta = \log{157.938.837}\}$, $p \in \{0.01, 0.02, \ldots, 0.99\}$.
        \item A chart of $\bar{\epsilon} \in \{40, 4, 1\}$ with three according convergence lines of the optimized parameters.
        \item A chart of objective value and best accuracy fixing $M = 1$, $\bar{\epsilon} = 4$, $l \in \{2^{\alpha x + \beta} | x \in [1, 1000], \alpha + \beta = 2, 1000 \alpha + \beta = \log{157.938.837}\}$, $p \in \{0.01, 0.02, \ldots, 0.99\}$.
        \item A chart of objective value and best accuracy fixing $M = 1$, $\bar{\epsilon} = 1$, $l \in \{2^{\alpha x + \beta} | x \in [1, 1000], \alpha + \beta = 2, 1000 \alpha + \beta = \log{157.938.837}\}$, $p \in \{0.01, 0.02, \ldots, 0.99\}$.
        \item A chart of objective value and best accuracy fixing $M = 1$, $\bar{\epsilon} = 0.1$, $l \in \{2^{\alpha x + \beta} | x \in [1, 1000], \alpha + \beta = 2, 1000 \alpha + \beta = \log{157.938.837}\}$, $p \in \{0.01, 0.02, \ldots, 0.99\}$.
        \item A chart of the maximum possible $\log(l + m)$ with variation of transmission power $P_k$ in range $[0.9, 1.8]$ GHz, given maximum transmission time $T = 5\times 10 ^ {-4}$ seconds. 
    \end{enumerate}

	\begin{frame}{Minimum privacy budget $\epsilon$ over maximal transmitting power $P_k^\max$ with different dimension number $d$. From left to right according to different bandwidth $W = $ 900, 1200, 1500 MHz.}
	   \begin{varwidth}{\textwidth}
	        \centering
	        \begin{figure}
	            \includegraphics{figures/minimum-privacy-budget-over-transmitting-power/min-eps-over-Pkmax-W900Mhz.png}
	            \caption{$W = 900 MHz$}
	            \label{fig:min-eps-over-Pkmax-W900Mhz}
	        \end{figure}
	   \end{varwidth}
	   \hfill
	\end{frame}
		
	In this paper, we consider the supervised distributed ML over a wireless network based on Mobile Edge Computing (MEC) architecture, illustrated in \cref{fig:1}, which consists of one Mobile Edge server and a set $\mathcal{K}$ of K mobile devices.
	The Mobile Edge server, which acts as a parameter server, orchestrates the learning process.
	
	\begin{table}[b]
		\caption {Notations}
		\label {table:1}
		\centering
		\begin{tabular}{|l|l|}
			\hline
			\textbf{Parameters}	&  \textbf{Description}													\\ \hline
			$l$					&  Level of quantization    											\\ \hline
			$m,p$				&  Parameter of Binomial Distribution   							\\ \hline
			$P_k$				&  The transmission power of node $n$  									\\ \hline
			$T$					&  Communication time  													\\ \hline
			$G$					&  Upper bound of gradient 												\\ \hline
			$s$					&  Noise scale												\\ \hline
			$\epsilon$,$\delta$ &  A parameter of $\left(\epsilon,\delta\right)$-Differential Privacy 	\\ \hline
			$K$					&  Number of devices													\\ \hline
			$\mathcal{K}$       &  Set of devices $\{1, 2, \ldots, K\}$                                 \\ \hline
			$d$					&  Dimension of data													\\ \hline
			$W$					&  Channel Bandwidth													\\ \hline
			$R_k$				&  Transmission rate of device $k$																	\\ \hline
			$N_0$				&  AWGN																	\\ \hline
			$\mathbb{N}$		&  Integer set 												\\ \hline
		\end{tabular}
		\\[10pt]
	\end{table}
	\subsection{Minimize the convergence time problem formulation}
	
	Due to the quantization and randomization, the obtained global gradient $\overline{\mathbf{g}}(\mathbf{w}^t)$ at the server is biased, i.e. $\mathbb{E}[\overline{\mathbf{g}}(\mathbf{w}^t)] - \nabla F(\mathbf{w}^t) \leq 2D\delta$ \cite{Agarwal2018}.
		
	From \eqref{eq:11}, the upper bound of $B'$ depends on the parameters $l,p,m$ of the mechanism $\mathcal{M}$.
	
	Finally, we consider the problem ($\mathscr{P}_2$) which is easier to solve than problem ($\mathscr{P}_1$). Moreover, the optimal solution of ($\mathscr{P}_2$) is also the optimal solution of ($\mathscr{P}_1$) as shown in Theorem \ref{relationship-P1-P2-models}. For the sake of simplicity, we also denote the objective function of ($\mathscr{P}_2$) as $f$ the same as the objective function of ($\mathscr{P}_1$).
	
	 We investigate the small value scenario for the differential privacy parameter $\bar{\epsilon}$ according respectively 4, 1 and 0.1. To ensure such a small value of $\bar{\epsilon}$, the feasible value $m$ is very large. If the number of devices is small, the learning algorithm is not stable. Hence, we only investigate this case with very large number of devices: $K = 10000$. The second scenario is with three values of $\epsilon$ as 50, 60 and 70. In this case, the learning algorithm is stable even with small number of devices and we investigate two cases: $K = 50$ and $K = 100$.
	 
	  Particularly, we study the case where $d = 47710$ as the number of weights of a typical implementation for artificial neuron networks for MNIST hand writing digits recognition with three layers including a hidden layer with 60 nodes \cite{Agarwal2018}.
	  
	   E.g., for the problem presented in the Section \ref{s:numerical-results}, $d = 47710$, $\delta = 10^{-10}$, $K = 100$ and $\bar{m}_\mathcal{M} = 2^8$, we have, $C \approx 1 / \eta \approx 30.831$ and $\lambda < \rho / 30.831 $.
	   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
BEGIN MINIMIZING THE PRIVACY BUDGET EPSILON UNDER THE SYSTEM CONSTRAINTS:
    \item 	What is the optimal differential privacy budget under the constraints of wireless networks?
    
    \section{Privacy budget minimizing problem}
	In this section, we investigate the problem of minimizing the privacy budget under the system constraints. First, we construct a model of this problem. The constraints are the same as the constraints of the Model ($\mathscr{P}_1$), but the objective function is the privacy budget. The model are as following:
	\begin{equation}
		(\mathscr{P}_3): \enspace \underset{l,m,p,P_k}{\mathrm{min}}\quad \epsilon(l,m,p,P_k) \label{md:min-eps-of}\\
	\end{equation}
	\begin{alignat}{2}
	    \hskip 1em \textrm{s.t.} \quad \eqref{eq:DP_cons}, \eqref{eq:channel_cap_cons}, \eqref{eq:trans_pow_cons}, \eqref{eq:domain_set_l_m} \ \text{and} \ \eqref{eq:domain_set_p}, \nonumber
	\end{alignat}
	where the formula of objective function $\epsilon(l,m,p,P_k)$ is defined by \eqref{eq:expression-epsilon}.
	
	The Theorem \ref{thrm:local-optimal-min-epsilon-model} states a result about the optimal solution of ($\mathscr{P}_3$) for a particular case where $0 < p \leq 1/2$.
	
	\begin{theorem} [Local Optimal solution of ($\mathscr{P}_3$) for particular case $p \leq 1/2$]
	\label{thrm:local-optimal-min-epsilon-model}
	    If ($\mathscr{P}_3$) has a feasible solution for $p \leq 1/2$, the following solution is the local optimal solution of ($\mathscr{P}_3$) for $p \in (0, 1/2]$:
	    \begin{align}
	        l^* &= \bar{l}_{\mathcal{L}}, \\
	        m^* &= (1 + \min_{k' \in \mathcal{K}} \frac{P^{\max}_{k'} h_{k'}}{N_0}) ^ {\frac{TW}{d}} - l^*, \\
	        p^* &= \frac{1}{2}, \\
	        P^*_k &= \max \{P_k^{\min}, \frac{\min_{k' \in \mathcal{K}} P^{\max}_{k'} h_{k'}}{h_k}\}, k \in \mathcal{K}.
	    \end{align}
	\end{theorem}
	\begin{proof}
	See Appendix \ref{proof-thrm-local-optimal-min-epsilon-model}.
	\end{proof}
		

	
	Figures \ref{fig:max-bits-nb-per-param-over-Pkmax-W900Mhz}, \ref{fig:max-bits-nb-per-param-over-Pkmax-W1200Mhz} and \ref{fig:max-bits-nb-per-param-over-Pkmax-W1500Mhz} present the maximal allowed number of transmit bits per parameter over the maximal transmit power. Each curve is corresponding to a particular dimension number, i.e., the number of parameters $d$. Each figure corresponds to a particular value of bandwidth. Here the upper bound of differential privacy budget $\bar{\epsilon} = 4$. As expected, as the maximal transmit power increases, the maximal number of transmit bits per parameter increases. As the bandwidth value increases, the maximal number transmit bits per parameter also increases.
	
	
	\begin{figure*}[!t]
	    \centering
	    \subfloat[$W = 900$ MHz] {\includegraphics[width=2.25in]{figures/minimum-privacy-budget-over-transmit-power/min-eps-over-Pkmax-W900Mhz.png}
    	\label{fig:min-eps-over-Pkmax-W900Mhz}}
    	\hfill
    	\subfloat[$W = 1200$ MHz]{\includegraphics[width=2.25in]{figures/minimum-privacy-budget-over-transmit-power/min-eps-over-Pkmax-W1200Mhz.png}%
    	\label{fig:min-eps-over-Pkmax-W1200Mhz}}
    	\hfill
    	\subfloat[$W = 1500$ MHz]{\includegraphics[width=2.25in]{figures/minimum-privacy-budget-over-transmit-power/min-eps-over-Pkmax-W1500Mhz.png}%
    	\label{fig:min-eps-over-Pkmax-W1500Mhz}}
    	\caption{Minimum privacy budget $\epsilon$ over maximal transmit power $E_k^\max$ with different dimension number $d$. From left to right according to different bandwidth $W = $ 900, 1200, 1500 MHz.}
    	\label{figs-group:min-eps-over-Pkmax-diff-bandwith}
	\end{figure*}
	
	  Figures \ref{fig:min-eps-over-Pkmax-W900Mhz}, \ref{fig:min-eps-over-Pkmax-W1200Mhz}, and \ref{fig:min-eps-over-Pkmax-W1500Mhz} present the logarithm of base 10 of the  minimum allowed privacy budget $\epsilon$ over the maximal transmit power in scenarios of bandwidths corresponding to 900, 1200, and 1500 MHz respectively. Here, we restrict the number of allowed transmit bits per parameter not exceeding 8 bits. These figures show that as the maximal transmit power increases the minimum allowed privacy budget gets smaller, i.e., the privacy security gets better. They also show that as the number of parameters gets larger, it is more difficult to guarantee privacy. Considering the bandwidths scenarios of 900, 1200 and 1500 MHz respectively, it is clear that as the bandwidth gets higher, it is easier to guarantee privacy.
 
	
     We also discussed about the problem of minimizing the privacy budget under the constraints of the mobile edge network. The achieved results relating to this problem are: \textit{(i)} A MIP model of the problem; \textit{(ii)} The formulas of optimal solution of the proposed MIP model in particular case whose the probability parameter of Binomial mechanism satisfying $0 < p \leq 1/2$. Since many questions relating to the minimizing privacy budget are remained, we intend to further investigate this problem.
    
    \section{Proof of the Theorem \ref{thrm:local-optimal-min-epsilon-model}}
	\label{proof-thrm-local-optimal-min-epsilon-model}
	For $p \in (0, 1/2]$, it is clear that, $b_p$, $c_p$ and $d_p$ are positive. Therefore, fixing $l$, $p$ and $P_k$, $\epsilon$ is decreasing by $m$. By \eqref{eq:channel_cap_cons}, we have,
	$$m \leq (1 + \frac{P_kh_k}{N_0})^{\frac{TW}{d}} - l, k \in \mathcal{K}.$$
	Since $P_k \leq P_k^{\max}$, we imply that,
	$$m \leq (1 + \min_{k' \in \mathcal{K}}\frac{P_{k'}^{\max}h_{k'}}{N_0})^{\frac{TW}{d}} - l.$$
	
	Since $\epsilon$ is decreasing by $m$ for $p \in (0, 1/2]$, if $$\tilde{m} &= (1 + \min_{k' \in \mathcal{K}} \frac{P^{\max}_{k'} h_{k'}}{N_0}) ^ {\frac{TW}{d}} - l,$$ then $\epsilon(l, m, p, P_k) \geq \epsilon(l, \tilde{m}, p, P_k)$ for $p \in (0, 1/2]$.
	
	In addition, since the left hand side expression of Constraint \eqref{eq:DP_cons} is increasing by $m$, then if $(l, m, p, P_k)$ satisfies \eqref{eq:DP_cons}, $(l, \tilde{m}, p, P_k)$ also satisfies \eqref{eq:DP_cons}. Hence, $m^*$ and $l^*$ of optimal solution for $p \in (0, 1/2]$ satisfy the formula
	$$m^* &= (1 + \min_{k' \in \mathcal{K}} \frac{P^{\max}_{k'} h_{k'}}{N_0}) ^ {\frac{TW}{d}} - l^*.$$
	
	Fixing $l$, $m$ and $P_k$, we could briefly write $\epsilon(l, m, p, P_k)$ as $\epsilon(p)$. We will prove that $\epsilon(p) \geq \epsilon(1/2)$ for $p \leq 1/2$. We could rewrite formulas \eqref{quadratic-form-bp-cp-dp} of $b_p$, $c_p$ and $d_p$ as followings,
	\begin{align}
	    b_p = \frac{4p(p - 1)}{3} + \frac{5 - 6p}{3}, c_p = 13\sqrt{2}p(p - 1) + 5\sqrt{2}, \nonumber\\
	    d_p = \frac{8p(p - 1)}{3} + \frac{4}{3}. \nonumber
	\end{align}
	We replace these formulations into places of $b_p$, $c_p$ and $d_p$ in \eqref{eq:expression-epsilon}, we have,
	\begin{align}
	    \epsilon =& \frac{\Delta_2\sqrt{2\log{\frac{1.25}{\delta}}}}{\sqrt{mp(1 - p)}} - \frac{13\sqrt{2}\Delta_2\sqrt{\log{\frac{10}{\delta}}}}{m(1 - \frac{\delta}{10})} + \nonumber\\
	    & \frac{5\sqrt{2}\Delta_2\sqrt{\log{\frac{10}{\delta}}}}{mp(1 - p)(1 - \frac{\delta}{10})} - \frac{4\Delta_1}{3m(1 - \frac{\delta}{10})} + \nonumber\\
	    & \frac{\Delta_1(5 - 6p)}{3mp(1 - p)(1 - \frac{\delta}{10})} + \frac{2\Delta_{\infty}\log{\frac{1.25}{\delta}}}{3mp(1 - p)} - \nonumber\\
	    & \frac{8\Delta_{\infty} \log{\frac{20d}{\delta}} \log{\frac{10}{\delta}}}{3m} + \frac{4\Delta_{\infty} \log{\frac{20d}{\delta}} \log{\frac{10}{\delta}}}{3mp(1 - p)}.
	\end{align}
    
    We group terms of $\epsilon$ into three groups as following,
    \begin{align}
        G(p)  =& \frac{\Delta_2\sqrt{2\log{\frac{1.25}{\delta}}}}{\sqrt{mp(1 - p)}} + \frac{5\sqrt{2}\Delta_2\sqrt{\log{\frac{10}{\delta}}}}{mp(1 - p)(1 - \frac{\delta}{10})} \nonumber + \\
        &  + \frac{2\Delta_{\infty}\log{\frac{1.25}{\delta}}}{3mp(1 - p)} + \frac{4\Delta_{\infty} \log{\frac{20d}{\delta}} \log{\frac{10}{\delta}}}{3mp(1 - p)}, \nonumber\\
        H(p) =& - \frac{13\sqrt{2}\Delta_2\sqrt{\log{\frac{10}{\delta}}}}{m(1 - \frac{\delta}{10})} - \frac{4\Delta_1}{3m(1 - \frac{\delta}{10})} - \nonumber \\
        & \frac{8\Delta_{\infty} \log{\frac{20d}{\delta}} \log{\frac{10}{\delta}}}{3m}, \nonumber\\
        I(p) =& \frac{\Delta_1(5 - 6p)}{3mp(1 - p)(1 - \frac{\delta}{10})}, \nonumber
    \end{align}
	here, $\epsilon(p) = G(p) + H(p) + I(p)$.
	
	Variable $p$ appears in denominators of terms of $G$ inside the quadratic form $p(1 - p)$. Since $p(1 - p) \leq 1/2(1 - 1/2)$ we have, $G(p) \geq G(1/2)$ for $p \in (0, 1/2]$.
	
	It is clear that, $H(p)$ does not change for $p \in (0, 1/2]$.
	
	Considering $I(p)$, we will prove that $I(p) \geq I(1/2)$ for $p \in (0, 1/2]$. We need to consider only $v(p) = (5 - 6p) / [p(1 - p)]$ for $p \in (0, 1/2]$. Take the derivative of $v(p)$, we have,
	$$\frac{dv(p)}{dp} = \frac{10 p - 5 - 6p^2}{p^2(1 - p)^2}.$$
	Since $10p - 5 - 6p^2 < 0$ for $p \in \mathbb{R}$, we imply that $v(p)$ is decreasing for $p \in \mathbb{R}$. Therefore, $I(p) \geq I(1/2)$ for $p \in (0, 1/2]$.
	
	As a sequence, we have: $\epsilon(p) \geq \epsilon(1/2)$ for $p \in (0, 1/2]$.
	
	We have, $Km1/2(1 - 1/2) \geq Kmp(1 - p)$, therefore if $(l, m, p, P_k)$ is a feasible solution of ($\mathscr{P}_3$) then $(l, m, 1/2, P_k)$ is also a feasible solution of ($\mathscr{P}_3$). Therefore, $p^* = 1/2$.
	
	Variable $l$ appears in $\Delta_1$, $\Delta_2$, $\Delta_{\infty}$ in the numerators of terms of $\epsilon$, it is clear that $\epsilon$ is decreasing by $l$ fixing $m$, $p$, $P_k$ for $p \in (0, 1/2]$. On the other hand, as $l^*$ gets smaller $m^*$ get larger. Therefore, $l^* = \min_\mathcal{M}$. 
	
	Finally, to save energy and to comply the Constraint \eqref{eq:trans_pow_cons}, we could assign $P_k^*$ as following,
	$$P^*_k &= \max \{P_k^{\min}, \frac{\min_{k' \in \mathcal{K}} P^{\max}_{k'} h_{k'}}{h_k}\}, k \in \mathcal{K}.$$
	
	The Theorem \ref{thrm:local-optimal-min-epsilon-model} is proved.

END MINIMIZING THE PRIVACY BUDGET EPSILON UNDER THE SYSTEM CONSTRAINTS:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Considering the Constraint \eqref{eq:channel_cap_cons}: $d\log_2(q^* + n^*) \leq TW\log_2(1 + E_k^*h_k/\omega_0)$ and constraints \eqref{eq:trans_pow_cons}: $E_k^{\min} \leq E_k^* \leq E_k^{\max}$, we imply that $d\log_2(q^* + n^*) \leq TW\log_2(1 + E_k^{\max}h_k/\omega_0)$. After transforming the last inequality, we have $n^* \leq (1 + \min_{k \in \mathcal{K}} E^{\max}_kh_k / \omega_0)^{TW / d} - q^*$. As a sequence, we have $n^* \leq (1 + \min_{k \in \mathcal{K}} E_k^*h_k/\omega_0)^{TW/d} - q^*$. Hence, $\mathcal{S}^*$ satisfies Constraint \eqref{eq:channel_cap_cons}.

\begin{figure*}[!t]
	    \centering
	    \subfloat[$W = 900$ MHz]{\includegraphics[width=2.25in]{figures/maximal-number-transmit-bits/max-bits-per-param-over-trans-power-W-900-MHz.png}%
    	\label{fig:max-bits-nb-per-param-over-Pkmax-W900Mhz}}
    	\hfill
    	\subfloat[$W = 1200$ MHz]{\includegraphics[width=2.25in]{figures/maximal-number-transmit-bits/max-bits-per-param-over-trans-power-W-1200-MHz.png}%
    	\label{fig:max-bits-nb-per-param-over-Pkmax-W1200Mhz}}
    	\hfill
    	\subfloat[$W = 1500$ MHz]{\includegraphics[width=2.25in]{figures/maximal-number-transmit-bits/max-bits-per-param-over-trans-power-W-1500-MHz.png}%
    	\label{fig:max-bits-nb-per-param-over-Pkmax-W1500Mhz}}
    	\caption{Maximal allowed number of transmit bits per parameter over maximal transmit power $P_k^\max$ ranging 1-20 dBm, with different dimension number $d$. From left to right according to different bandwidth $W = $ 900, 1200, 1500 MHz.}
    	\label{figs-group:max-bits-nb-per-param-over-Pkmax-diff-bandwith}
	\end{figure*}
	
	Figures \ref{fig:max-bits-nb-per-param-over-Pkmax-W900Mhz}, \ref{fig:max-bits-nb-per-param-over-Pkmax-W1200Mhz} and \ref{fig:max-bits-nb-per-param-over-Pkmax-W1500Mhz} present the maximal allowed number of transmit bits per parameter over the maximal transmit power. Each curve is corresponding to a particular dimension number, i.e., the number of parameters $d$. Each figure corresponds to a particular value of bandwidth. Here the upper bound of differential privacy budget $\bar{\epsilon} = 4$. As expected, as the maximal transmit power increases, the maximal number of transmit bits per parameter increases. As the bandwidth value increases, the maximal number transmit bits per parameter also increases.
